A Structural Approach to the Design of Domain Specific Neural Network Architectures

This is a master's thesis concerning the theoretical ideas of geometric deep learning. Geometric deep learning aims to provide a structured characterization of neural network architectures, specifically focused on the ideas of invariance and equivariance of data with respect to given transformations. This thesis aims to provide a theoretical evaluation of geometric deep learning, compiling theoretical results that characterize the properties of invariant neural networks with respect to learning performance.

==> kapitel/bibliography.tex <==
\bibliographystyle{plain}
\bibliography{../literatur/diplom}

==> kapitel/erklaerung.tex <==
% erklaerung.tex
\cleardoublepage
\normalsize
Hiermit versichere ich, dass ich die vorliegende Arbeit selbstständig verfasst habe und keine anderen als die angegebenen Quellen und Hilfsmittel verwendet sowie Zitate kenntlich gemacht habe.\\\\
Dortmund, den \today \\\\\\\\
Gerrit Nolte% EOF

\begin{figure}[htbp]
\centerline{\includegraphics[scale=.9]{bilder/eiddesstatt.png}}
\end{figure}
